PrefixQuant: Eliminating Outliers by Prefixed Tokens for Large Language Models Quantization

Existing weight-activation quantization methods for Large Language Models (LLMs) primarily address channel-wise outliers but often neglect token-wise outliers, which limits the accuracy of quantized models. In this work, we propose PrefixQuant, a novel quantization method that achieves state-of-the-art performance across various precision levels (W4A4KV4 and W4A8KV4) and granularities (dynamic and static quantization) by effectively isolating token-wise outliers. First, PrefixQuant eliminates token-wise outliers by prefixing outlier tokens in the KV cache, a process that is training-free and highly efficient (e.g., 1 minutes for Llama-3-70B). Second, PrefixQuant introduces new trainable parameters for block-wise training to compensate for quantization error. Our experiments show that PrefixQuant significantly outperforms existing dynamic quantization methods, even under coarser static quantization settings. For instance, PrefixQuant achieves an average accuracy improvement of +3.08 and +2.85 points over SpinQuant (dynamic quantization) on five zero-shot reasoning tasks under dynamic and static quantization settings, respectively, on W4A4KV4 Llama-3-8B. Additionally, we demonstrate up to 2.74x prefilling speedup and 2.16x decoding speedup for LLMs using W4A4 PrefixQuant. Our code is available at https://github.com/ChenMnZ/PrefixQuant.

==> figure_text/framework.tex <==
% \begin{figure}[htbp]
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/framework_original.pdf}
        \vspace{-0.7em}
        \caption{Original}
        \label{fig:framework_origin}
    \end{subfigure}
    % \hfill
    \hspace{10pt}
    \begin{subfigure}[b]{0.4\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/framework_prefixquant.pdf}
        \vspace{-0.7em}
        \caption{PrefixQuant}
        \label{fig:framework_prefixquant}
    \end{subfigure}
    \hfill
    \caption{\textbf{Comparison of Original and PrefixQuant Inference.} Both methods use Hadamard rotation to remove channel-wise outliers. PrefixQuant differs by setting specific prefixed tokens in the KV cache, which eliminates token-wise outliers in linear inputs and $\mathbf{Q}$/$\mathbf{K}$/$\mathbf{V}$, enhancing compatibility with per-tensor static quantization. Llama-2-7B serves as an example; additional prefixed tokens for other models are listed in Table~\ref{tab:prefixed_token}.}
    \label{fig:framework}
\end{figure}


==> figure_text/lower_outlier.tex <==
% \begin{figure}[htbp]
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/lower_outlier/llama-2-7b-apply_rotary_pos_emb_qk_rotation_wrapper.K.pdf}
        \vspace{-0.7em}
        \caption{Original}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/lower_outlier/llama-2-7b-apply_rotary_pos_emb_qk_rotation_wrapper.K-rotate.pdf}
        \vspace{-0.7em}
        \caption{w/ Hadamard rotation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/lower_outlier/llama-2-7b-apply_rotary_pos_emb_qk_rotation_wrapper.K-prefixquant.pdf}
        \vspace{-0.7em}
        \caption{PrefixQuant}
    \end{subfigure}
    \caption{\textbf{Lower outliers in $\mathbf{K}$ of self-attention mechanism in LLaMA-2-7B}. Same setting as Figure~\ref{fig:upper_outlier_example}  }
    \label{fig:upper_outlier_example}
\end{figure}


==> figure_text/upper_outlier.tex <==
% \begin{figure}[htbp]
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/upper_outlier/llama-2-7b-down_proj.pdf}
        \vspace{-0.7em}
        \caption{Original}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/upper_outlier/llama-2-7b-down_proj-rotate.pdf}
        \vspace{-0.7em}
        \caption{w/ Hadamard rotation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \centering
        \includegraphics[width=\textwidth]{figures/upper_outlier/llama-2-7b-down_proj-prefixquant.pdf}
        \vspace{-0.7em}
        \caption{PrefixQuant}
    \end{subfigure}
    \caption{\textbf{Upper outliers in the inputs of the down\_proj linear layers in LLaMA-2-7B}. 
    Top-1, Medium, Min-1 indicate the largest, median, and smallest token-wise maximum values, respectively. We also calculate the the ratios of $\frac{\text{Top-1}}{\text{Median}}$ and $\frac{\text{Median}}{\text{Min-1}}$ in each layer, and report the maximum ratio.  Lower ratio indicate more uniform distribution. }
    \label{fig:upper_outlier_example}
\end{figure}


==> tables/ablation_dataset_with_acc.tex <==
\begin{table}[!ht]
\renewcommand{\tabcolsep}{1pt}
\centering
    \caption{Ablation studies on calibration dataset, including (a) Dataset type, (b) Training sequence length and (c) Total training tokens. ``N'' indicates number of training samples, and ``S'' is the length of each samples. The model used here is Llama-3-8B with w4a4kv4 quantization. Our default settings are marked in {\setlength{\fboxsep}{2pt}\colorbox{mygray}{{gray}}}.}
\begin{subtable}[b]{0.30\linewidth}
    \centering
    \subcaption{Dataset}
    \begin{tabular}{ccc}
    \toprule
    Dataset & Wiki PPL & Avg. Acc. \\
    \midrule
    C4 & 7.60 & -\\
    RedPajama & 7.49 & - \\
    \cellcolor{mygray}Pile & \textbf{7.42} & \textbf{71.08} \\
    \bottomrule
    \end{tabular}
\end{subtable}
\hspace{10pt}
\begin{subtable}[b]{0.30\linewidth}
    \centering
    \subcaption{Sequence length}
    \begin{tabular}{ccc}
    \toprule
    N $\times$ S & Wiki PPL & Avg. Acc. \\
    \midrule
    256 $\times$2048 & 7.65 & - \\
    \cellcolor{mygray}512$\times$1024 & \textbf{7.42} & \textbf{71.08} \\
    1024$\times$512 & 7.65 & - \\
    \bottomrule
    \end{tabular}
\end{subtable}
\hspace{10pt}
\begin{subtable}[b]{0.30\linewidth}
    \centering
    \subcaption{Total token number}
    \begin{tabular}{ccc}
    \toprule
    N $\times$ S & Wiki PPL & Avg. Acc. \\
    \midrule
    256 $\times$1024 & 7.46 & - \\
    \cellcolor{mygray}512 $\times$1024 & 7.42 & \textbf{71.08} \\
    1024$\times$1024 & 7.41 & - \\
    \bottomrule
    \end{tabular}
\end{subtable}

\end{table}

==> tables/ablation_dynamic.tex <==
\begin{table}[!t]
    \centering
    \caption{Ablation study about quantization type of activation. The model used here is Llama-3-8B with W4A4KV4 quantization. WikiText2 perplexity with 2048 context length is reported.}
    \begin{tabular}{ccccc}
    \toprule
    \bf{Fine-Tuning} & \bf{Quant Type} & \bf{W4A8KV4} & \bf{W4A4KV4} \\
    \midrule
    No & token-wise dynamic & \textbf{6.84} & 8.29 \\
    No & tensor-wise static & 6.90 & \textbf{7.93} \\
    Yes & token-wise dynamic & \textbf{6.60} & 7.88 \\
    Yes & tensor-wise static & 6.63 & \textbf{7.41} \\
    \bottomrule
    \end{tabular}
    \label{tab:ablation_dynamic}
\end{table}


% \begin{table}[!ht]
%     \centering
%     \caption{Ablation study about quantization type of activation. The model used here is Llama-3-8B with W4A4KV4 quantization.}
%     \begin{tabular}{cccc}
%     \toprule
%     Fine-Tuning & Quant Type & Wiki PPL \\
%     \midrule
%     No & token-wise dynamic & 8.29 \\
%     No & tensor-wise static & \textbf{7.93} \\
%     Yes & token-wise dynamic & 7.88 \\
%     Yes & tensor-wise static & \textbf{7.41} \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:ablation_dynamic}
% \end{table}

==> tables/e2e_prefilling_3_8b_a100.tex <==
% \begin{table}[!ht]
\begin{figure}[!h]
    \centering
    \setlength\tabcolsep{3pt}
    \renewcommand{\arraystretch}{0.5}
    \caption{Inference speedup of W4A4 Llama-2-7B model over the FP16 model on RTX 3090 GPU. For prefilling, we report the latency to deal with 2048 input tokens. For decoding, we report the token generation speed of generate 256 new tokens with 2048 prefillinng length. }
    \begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}{Method} & prefilling & decoding \\
    & (ms) & (token/s) \\
    \midrule
    \multicolumn{3}{c}{batch size = 1} \\
    \cdashline{1-3}
    FP16 & 162 & 62 \\
    PrefixQuant-O1 (W4A4) & 104 & 90 \\
    PrefixQuant-O2 (W4A4)& 100 (\bf{1.6x}) & 92 (\textbf{1.5x}) \\
    \midrule
    \multicolumn{3}{c}{batch size =4} \\
    \cdashline{1-3}
    FP16 & 621 & 190 \\
    PrefixQuant-O1 (W4A4) &  383 & 252 \\
    PrefixQuant-O2 (W4A4) & 371 (\bf{1.7x}) & 250 \textbf{(1.5x)} \\
    \bottomrule
    \end{tabular}
    \label{tab:e2e_prefilling}
% \end{table}
\end{figure}


% % \begin{table}[!ht]
% \begin{figure}[!h]
%     \centering
%     \setlength\tabcolsep{1.5pt}
%     \renewcommand{\arraystretch}{0.4}
%     \caption{Time-to-first-token (prefilling) speedup of W4A4 Llama-3-8B model over the FP16 model. We use 2048 sequence length with different batch size. }
%     \begin{tabular}{rll}
%     \toprule
%     Batchsize & 1 & 4 \\
%     \midrule
%     \multicolumn{3}{c}{on a RTX 3090 GPU (ms)} \\
%     \cdashline{1-3}
%     FP16 & 509 & OOM \\
%     Quarot (W4A4) & 221 (2.30x) & 851 \\
%     PrefixQuant (W4A4) & 181 (\bf{2.81x}) & \textbf{725} \\
%     \midrule
%     \multicolumn{3}{c}{on an A100-80GB GPU (ms)} \\
%     \cdashline{1-3}
%     FP16 & 172 & 661\\
%     Quarot (W4A4) &  130 (1.31x)& 477 (1.39x) \\
%     PrefixQuant (W4A4) & 107 (\bf{1.60x}) & 362 (\bf{1.82x})\\
%     \bottomrule
%     \end{tabular}
%     \label{tab:e2e_prefilling}
% % \end{table}
% \end{figure}

==> tables/plug_and_play.tex <==
\begin{table}[!ht]
    \centering
    \caption{Plug-and-play experiments. We combine existing methods with the proposed prefixed outlier in KV cache. ``PPL'' indicates WikiText2 perplexity measured with context length 2048.}
    \begin{tabular}{cccc}
    \toprule
    Model & Precision & Method  & PPL. \\
    \midrule
    & W4A4KV4 & QuaRot & - 
    &  &
         &  \\
         & 
    \bottomrule
    \end{tabular}
    \label{tab:plug_and_play_results}
\end{table}

==> tables/qlinear_comparisons.tex <==
\begin{table}[!ht]
    \caption{Speedup of W4A4 quantized linear layers compared to FP16 linear layer. Numbers in brackets indicate the speedup compared to FP16.}
    \centering
\begin{subtable}[b]{\linewidth}
\centering
 \subcaption{\textbf{Nvidia RTX 3090 GPU}}
    \begin{tabular}{cclll}
    \toprule
     \multirow{2}{*}{\textbf{(Seq\_len,input\_c, output\_c)}} & \multirow{2}{*}{\textbf{FP16} (ms)} & \multicolumn{3}{c}{\textbf{W4A4} (ms)} \\
     \cmidrule(lr){3-5}
   & & Quarot & + static quant & + improved GEMV \\
     \midrule
     (1,4096,4096) & 0.0512 & 0.0578 (0.89x) & 0.0472 (1.08x) & 0.0223 (\textbf{2.30x}) \\
     (1,4096,14336) & 0.1548 & 0.0641 (2.42x) & 0.0549 (2.83x) & 0.0475 (\textbf{3.27x}) \\
     (1,8192,8192) & 0.1080 & 0.0957 (1.77x) &  0.0863 (1.97x) & 0.0561 (\textbf{3.02x}) \\
     (1,8192,28672) & 0.5762 & 0.2087 (2.76x) & 0.1977 (2.91x) & 0.1503 (\textbf{3.83x}) \\
     (2048,4096,4096) & 1.0666 & 0.3699 (2.88x) &  0.2965 (\textbf{3.59x}) &-\\
     (2048,4096,14336) & 3.5766 & 0.9358 (3.93x) & 0.8618 (\textbf{4.27x}) & -\\
     (2048,8192,8192) & 3.9986 & 1.0211 (4.03x) & 0.8718 (\textbf{4.72x}) & -\\
     (2048,8192,28672) & 13.1607 &  2.8609 (4.74x) & 2.7177 (\textbf{4.99x}) & -\\
     \bottomrule
    \end{tabular}
\end{subtable}
\begin{subtable}[b]{\linewidth}
\centering
 \subcaption{\textbf{Nvidia A100-80GB GPU}}
    \begin{tabular}{cclll}
    \toprule
     \multirow{2}{*}{\textbf{(Seq\_len,input\_c, output\_c)}} & \multirow{2}{*}{\textbf{FP16} (ms)} & \multicolumn{3}{c}{\textbf{INT4} (ms)} \\
     \cmidrule(lr){3-5}
   & & Quarot & + static quant & + improved GEMV \\
     \midrule
     (1,4096,4096) & 0.0418 & 0.0588 (0.71x) & 0.0455 (0.92x) & 0.0235 (\textbf{1.78x}) \\
     (1,4096,14336) & 0.1026 & 0.0679 (1.51x) & 0.0556 (1.85x) & 0.0441 (\textbf{2.33x}) \\
     (1,8192,8192) & 0.1080 & 0.0888 (1.22x) & 0.0735 (1.47x) & 0.0508 (\textbf{2.13x}) \\
     (1,8192,28672) & 0.3036 & 0.1668 (1.82x) & 0.1534 (1.97x) & 0.1114 (\textbf{2.72x})\\
     (2048,4096,4096) & 0.2762 & 0.2408 (1.15x) & 0.1799 (\textbf{1.54x}) & -\\
     (2048,4096,14336) & 1.0092 & 0.5461 (1.85x) & 0.4850 (\textbf{2.08x}) & -\\
     (2048,8192,8192) & 1.0583 & 0.5298 (2.00x) & 0.4349 (\textbf{2.43x})& -\\
     (2048,8192,28672) & 3.6897 & 1.4686 (2.51x) & 1.3857 (\textbf{2.66x}) & -\\
     \bottomrule
    \end{tabular}
\end{subtable}
    \label{tab:qlinear_comparisons}
\end{table}

==> tables/qlinear_comparsions_2.tex <==
\begin{table}[!h]
    \caption{Speedup of quantize linear layers. Numbers in brackets indicate the speedup compared to FP16.}
    \centering
\begin{subtable}[b]{\linewidth}
\centering
 \subcaption{\textbf{Nvidia RTX 3090 GPU}}
    \begin{tabular}{cclll}
    \toprule
     \multirow{2}{*}{\textbf{(Seq\_len,input\_c, output\_c)}} & \multirow{2}{*}{\textbf{FP16} (ms)} & \multicolumn{3}{c}{\textbf{INT4} (ms)} \\
     \cmidrule(lr){3-5}
   & & Quarot & + static quant & + improved GEMV \\
     \midrule
     (1,4096,4096) & 0.0512 & 0.0578 (0.89x) & 0.0472 (1.08x) & 0.0223 (\textbf{2.30x}) \\
     (1,4096,14336) & 0.1548 & 0.0641 (2.42x) & 0.0549 (2.83x) & 0.0475 (\textbf{3.27x}) \\
     (1,8192,8192) & 0.1080 & 0.0957 (1.77x) &  0.0863 (1.97x) & 0.0561 (\textbf{3.02x}) \\
     (1,8192,8192) & 0.1080 & 0.0957 (1.77x) &  0.0863 (1.97x) & 0.0561 (\textbf{3.02x}) \\
     (1,8192,28672) & 0.5762 & 0.2087 (2.76x) & 0.1977 (2.91x) & 0.1503 (\textbf{3.83x}) \\
     (2048,4096,4096) & 1.0666 & 0.3699 (2.88x) &  0.2965 (\textbf{3.59x}) &-\\
     (2048,4096,14336) & 3.5766 & 0.9358 (3.93x) & 0.8618 (\textbf{4.27x}) & -\\
     (2048,8192,8192) & 3.9986 & 1.0211 (4.03x) & 0.8718 (\textbf{4.72x}) & -\\
     (2048,8192,28672) & 13.1607 &  2.8609 (4.74x) & 2.7177 (\textbf{4.99x}) & -\\
     \bottomrule
    \end{tabular}
\end{subtable}
\begin{subtable}[b]{\linewidth}
\centering
 \subcaption{\textbf{Nvidia A100-80GB GPU}}
    \begin{tabular}{cclll}
    \toprule
     \multirow{2}{*}{\textbf{(Seq\_len,input\_c, output\_c)}} & \multirow{2}{*}{\textbf{FP16} (ms)} & \multicolumn{3}{c}{\textbf{INT4} (ms)} \\
     \cmidrule(lr){3-5}
   & & Quarot & + static quant & + improved GEMV \\
     \midrule
     (1,4096,4096) & 0.0418 & 0.0588 (0.71x) & 0.0455 (0.92x) & 0.0235 (\textbf{1.78x}) \\
     (1,4096,14336) & 0.1026 & 0.0679 (1.51x) & 0.0556 (1.85x) & 0.0441 (\textbf{2.33x}) \\
     (1,8192,8192) & 0.1080 & 0.0888 (1.22x) & 0.0735 (1.47x) & 0.0508 (\textbf{2.13x}) \\
     (1,8192,28672) & 0.3036 & 0.0888 (1.22x) & 0.0735 (1.47x) & 0.0508 (\textbf{2.13x})\\
     (2048,4096,4096) & 0.2762 & 0.2408 (1.15x) & 0.1799 (\textbf{1.54x}) & -\\
     (2048,4096,14336) & 1.0092 & 0.5461 (1.85x) & 0.4850 (\textbf{2.08x}) & -\\
     (2048,8192,8192) & 1.0583 & 0.5298 (2.00x) & 0.4349 (\textbf{2.43x})& -\\
     (2048,8192,28672) & 3.6897 & 1.4686 (2.51x) & 1.3857 (\textbf{2.66x}) & -\\
     \bottomrule
    \end{tabular}
\end{subtable}
    \label{tab:qlinear_comparisons}
\end{table}

==> tables/quantitative.tex <==
% \renewcommand \arraystretch{1.05}
\begin{table*}[t]
\renewcommand{\arraystretch}{0.4}
    \setlength{\tabcolsep}{2pt}
    % \small
    \centering
    \vspace{5pt}
    \begin{tabular}{lccccccc}
        \toprule
          \multirow{2}{*}{\textbf{PPL $\downarrow$}}   & \multirow{2}{*}{\bf{FP16}}  & \multicolumn{3}{c}{\bf{W16A4KV16 (static)}}  & \multicolumn{3}{c}{\bf{W16A16KV4 (static)}}  \\ 
          \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
         &  & original & + rotation & + prefixed &   original & + rotation & + prefixed    \\
         \midrule
         Llama-2-7B & 5.47 & 3024.77 & 17.95 & \textbf{5.91} & 6.46 & 5.95 & \textbf{5.56} \\
         Llama-3-8B & 6.14 & 1816.57 & 22.14 & \textbf{7.23} & 7.37 & 8.12 & \textbf{6.30} \\
        \bottomrule
    \end{tabular}
    \caption{ Proposed prefixed outliers in KV cache significantly improves the performance of the static quantized models over hadamard rotation~\cite{quarot,spinquant}. W16A4KV16 indicates 4-bit per-tensor static quantization of all linear layer inputs. W16A16KV4 indicates 4-bit per-head static KV cache quantization. WikiText2 perplexity with 2048 context length is reported.
    } 
    \label{tab:teaser}
\end{table*}


==> tables/quantization_setting_2.tex <==
\begin{table}[!h]
    \centering
    \setlength{\tabcolsep}{0.5pt}
    \caption{Detailed quantization setting of comparison methods. All per-group quantization set group size as 128.}
    \label{tab:quantization_settngs}
    \begin{tabular}{cccc}
    \toprule
    \bf{Method} & \bf{Weight} & \bf{Activation} & \bf{KV Cache} \\
    \midrule
    SmoothQuant & per-channel symmetric & per-token symmetric dynamic &  per-tensor symmetric static \\
    Atom &  per-group symmetric & per-group symmetric dynamic & per-group asymmetric dynamic \\
    QoQ & per-channel asymmetric & per-token symmetric dynamic & per-group asymmetric dynamic\\
    QuaRot & per-channel symmetric & per-token dynamic symmetric & per-group asymmetric dynamic \\
    DuQuant & per-channel asymmetric & per-token dynamic asymmetric & per-token asymmetric dynamic \\
    \textbf{\methodshort} & per-channel symmetric & per-tensor symmetric static & per-head  symmetric static\\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/static_vs_dynamic_quant.tex <==
\begin{table}[!ht]
    \centering
    \caption{Speedup of per-tensor static quantization compared to per-token dynamic quantization in 4-bit activation quantization. }
\begin{subtable}[b]{0.9\linewidth}
\centering
    \subcaption{\textbf{Nvidia RTX 3090 GPU}}
    \begin{tabular}{cccc}
    \toprule
    \multirow{2}{*}{\textbf{(Seq\_len,dimension)}} & \multicolumn{2}{c}{\textbf{Quantization Time} (ms)} & \multirow{2}{*}{\textbf{Speedup}} \\
    \cmidrule(lr){2-3}
    & \textbf{Per-token Dynamic} & \textbf{Per-tensor static} & \\
    \midrule
    (1,4096) & 0.0127 & 0.0038 & 3.34x \\
    (1,8192) & 0.0144 & 0.004 & 3.60x \\
    (2048,4096) & 0.1073 & 0.0344 & 3.12x \\
    (2048,8192) & 0.2084 & 0.0652 & 3.19x \\
    \midrule
    \textbf{Average Speedup} & & & \textbf{3.31x} \\
    \bottomrule
    \end{tabular}
\end{subtable}
\begin{subtable}[b]{0.9\linewidth}
\centering
    \subcaption{\textbf{Nvidia A100-80GB GPU}}
    \begin{tabular}{cccc}
    \toprule
    \multirow{2}{*}{\textbf{(Seq\_len,dimension)}} & \multicolumn{2}{c}{\textbf{Quantization Time} (ms)} & \multirow{2}{*}{\textbf{Speedup}} \\
    \cmidrule(lr){2-3}
    & \textbf{Per-token Dynamic} & \textbf{Per-tensor static} & \\
    \midrule
    (1,4096) & 0.020 & 0.0072 & 2.81x \\
    (1,8192) & 0.022 & 0.0075 & 2.88x \\
    (2048,4096) & 0.095 & 0.033 & 2.88x \\
    (2048,8192) & 0.157 & 0.058 & 2.71x \\
    \midrule
    \textbf{Average Speedup} & & & \textbf{2.82x} \\
    \bottomrule
    \end{tabular}
\end{subtable}

    \label{tab:static_vs_dynamic_quant}
\end{table}

==> tables/w8a8kv8.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{0.6}
\centering
\caption{W8A8KV8 results. Refer Table~\ref{tab:w4a4} for the metric setting and performance of full-precision models.}
\label{tab:w8a8}
\begin{tabular}{ccccc}
\toprule
\bf{Model} & \bf{Method} & \bf{Quant Type} & \bf{Wiki} \bf{PPl} & \bf{Avg. Acc.} \\
\midrule
\multirow{4}{*}{Llama-2-7B} & SmoothQuant & dynamic & 5.54 & 68.92\\
& QuaRot & dynamic & \textbf{5.48} & \textbf{69.11} \\
& \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} \textbf{5.48}  & \cellcolor{mylightblue} 68.97 \\
\midrule
\multirow{3}{*}{Llama-2-13B} & SmoothQuant & dynamic & 4.95 & 71.58 \\
& QuaRot & dynamic & \textbf{4.89} & \textbf{71.69} \\
& \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} \textbf{4.89}  & \cellcolor{mylightblue} 71.52 \\
\midrule
\multirow{3}{*}{Llama-2-70B} & SmoothQuant & dynamic & 3.36 & 76.19 \\
& QuaRot & dynamic & \textbf{3.32} & \textbf{76.53} \\
& \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 3.39  & \cellcolor{mylightblue} 76.11 \\
\midrule
\multirow{3}{*}{Llama-3-8B} & SmoothQuant & dynamic & 6.28 & 72.73 \\
& QuaRot & dynamic & \textbf{6.15} & 72.77 \\
& \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 6.17  & \cellcolor{mylightblue} \textbf{73.10} \\
\midrule
\multirow{3}{*}{Llama-3-70B} & SmoothQuant & dynamic & 3.26 & 79.29 \\
& QuaRot & dynamic & \textbf{2.90} & \textbf{79.83} \\
& \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 2.93  & \cellcolor{mylightblue} 78.61 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/w8a8kv8_and_w4a8kv4.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{0.6}
\centering
\caption{W8A8KV8 and W4A8KV4 results. Refer Table~\ref{tab:w4a4} for the metric setting and performance of full-precision models.}
\label{tab:w8a8_and_w4a8}

\begin{subtable}[b]{0.9\linewidth}
\centering
    \subcaption{\textbf{W8A8KV8 results.}}\label{tab:w8a8}
    \begin{tabular}{ccccc}
    \toprule
    \bf{Model} & \bf{Method} & \bf{Quant Type} & \bf{Wiki} \bf{PPl} & \bf{Avg. Acc.} \\
    \midrule
    \multirow{4}{*}{Llama-2-7B} & SmoothQuant & dynamic & 5.54 & 68.92\\
    & QuaRot & dynamic & \textbf{5.48} & \textbf{69.11} \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} \textbf{5.48}  & \cellcolor{mylightblue} 68.97 \\
    \midrule
    \multirow{3}{*}{Llama-2-13B} & SmoothQuant & dynamic & 4.95 & 71.58 \\
    & QuaRot & dynamic & \textbf{4.89} & \textbf{71.69} \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} \textbf{4.89}  & \cellcolor{mylightblue} 71.52 \\
    \midrule
    \multirow{3}{*}{Llama-2-70B} & SmoothQuant & dynamic & 3.36 & 76.19 \\
    & QuaRot & dynamic & \textbf{3.32} & \textbf{76.53} \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 3.39  & \cellcolor{mylightblue} 76.11 \\
    \midrule
    \multirow{3}{*}{Llama-3-8B} & SmoothQuant & dynamic & 6.28 & 72.73 \\
    & QuaRot & dynamic & \textbf{6.15} & 72.77 \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 6.17  & \cellcolor{mylightblue} \textbf{73.10} \\
    \midrule
    \multirow{3}{*}{Llama-3-70B} & SmoothQuant & dynamic & 3.26 & 79.29 \\
    & QuaRot & dynamic & \textbf{2.90} & \textbf{79.83} \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 2.93  & \cellcolor{mylightblue} 78.61 \\
    \bottomrule
    \end{tabular}
\end{subtable}

\begin{subtable}[b]{0.9\linewidth}
\centering
    \subcaption{\textbf{W4A8KV4 results.}}\label{tab:w4a8}
    \begin{tabular}{ccccc}
    \toprule
    \bf{Model} & \bf{Method} & \bf{Activation Quant} & \bf{Wiki PPl} &  \bf{Avg. Acc.} \\
    \midrule
    \multirow{6}{*}{Llama-2-7B} & QoQ & dynamic & 5.75 &  67.22 \\
    & QuaRot & dynamic & 5.73  & 67.11 \\
    % & QoQ & static & \\
    % & QuaRot & static & \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 5.76  & \cellcolor{mylightblue} 67.86 \\
    & \cellcolor{mylightblue} \methodshort & \cellcolor{mylightblue} static & \cellcolor{mylightblue} \textbf{5.68}  & \cellcolor{mylightblue} \textbf{68.90} \\
    \midrule
    \multirow{4}{*}{Llama-2-13B} & QoQ & dynamic & 5.12 & 70.56 \\
    & QuaRot & dynamic & 5.07  & 69.96 \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 5.08  & \cellcolor{mylightblue} 71.07 \\
    & \cellcolor{mylightblue} \methodshort & \cellcolor{mylightblue} static & \cellcolor{mylightblue} \textbf{5.07}  & \cellcolor{mylightblue} \textbf{71.25} \\
    \midrule
    \multirow{4}{*}{Llama-2-70B} & QoQ & dynamic & 3.52  & 75.91 \\
    & QuaRot & dynamic & 3.46  & 76.31 \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 3.60 & \cellcolor{mylightblue} 75.00 \\
    & \cellcolor{mylightblue} \methodshort & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 3.50 & \cellcolor{mylightblue} 76.50 \\
    \midrule
    \multirow{4}{*}{Llama-3-8B} & QoQ & dynamic & 6.89  & 71.35 \\
    & QuaRot & dynamic & 6.80  & 71.68 \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 6.90 & \cellcolor{mylightblue} 70.29 \\
    & \cellcolor{mylightblue} \methodshort & \cellcolor{mylightblue} static & \cellcolor{mylightblue} \textbf{6.62}  & \cellcolor{mylightblue} \textbf{72.46} \\
    \midrule
    \multirow{4}{*}{Llama-3-70B} & QoQ & dynamic & 4.36 & 78.12 \\
    & QuaRot & dynamic & 3.73 & \textbf{78.92} \\
    & \cellcolor{mylightblue} \methodshort w/o FT & \cellcolor{mylightblue} static & \cellcolor{mylightblue} 3.55 & \cellcolor{mylightblue} 77.82 \\
    & \cellcolor{mylightblue} \methodshort & \cellcolor{mylightblue} static & \cellcolor{mylightblue} \textbf{3.43} & \cellcolor{mylightblue} 78.70 \\
    \bottomrule
    \end{tabular}
\end{subtable}



\end{table}

==> tables/weight-only.tex <==
%[TODO] add AQLM and QUIP#
\begin{table}[!ht]
\renewcommand{\arraystretch}{0.4}
    \centering
    \caption{Weight-only quantization results. ``g'' indicates group size for weight quantization.}
    \label{tab:weight-only}
\begin{subtable}[b]{0.9\linewidth}
    \subcaption{\bf{Llama-3-8B results.}}
    \begin{tabular}{ccccc}
    \toprule
    Llama-3-8B & \multicolumn{2}{c}{W3A16g128} & \multicolumn{2}{c}{W2A16g128} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    FP (Wiki PPL:6.14; Avg. Acc:72.61)& Wiki & Avg. Acc. & Wiki & Avg. Acc. \\
    \midrule
    EfficientQAT (w/o E2E-QP) & 7.34
     & 70.80 & 13.55  & 58.95 \\
    \rowcolor{mylightblue} \methodshort & 7.17 & 72.10 & 11.93 & 64.00 \\
    % EfficientQAT (w/ E2E-QP) & \\
    % \rowcolor{mylightblue} \methodshort (w/ E2E-QP) & \\
    \bottomrule
    \end{tabular}
    \label{tab:weight-only-llama-3-8b}
\end{subtable}

\begin{subtable}[b]{0.9\linewidth}
    \subcaption{\bf{Llama-3-70B results.}}
    \begin{tabular}{ccccc}
    \toprule
    Llama-3-70B & \multicolumn{2}{c}{W3A16g128} & \multicolumn{2}{c}{W2A16g128} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
    FP (Wiki PPL:2.85; Avg. Acc:80.03)& Wiki & Avg. Acc. & Wiki & Avg. Acc. \\
    \midrule
    EfficientQAT (w/o E2E-QP) &4.89 & 75.65 & 16.79 & 67.88\\
    \rowcolor{mylightblue} \methodshort & 4.79 & 77.75 & 11.01 & 72.61 \\
    % EfficientQAT (w/ E2E-QP) & \\
    % \rowcolor{mylightblue} \methodshort (w/ E2E-QP) & \\
    \bottomrule
    \end{tabular}
    \label{tab:weight-only-llama-3-70b}
\end{subtable}
\end{table}
